Early Performance Prediction using Interpretable Patterns in Programming Process Data

Instructors have limited time and resources to help struggling students, and these resources should be directed to the students who most need them. To address this, researchers have constructed models that can predict students' final course performance early in a semester. However, many predictive models are limited to static and generic student features (e.g. demographics, GPA), rather than computing-specific evidence that assesses a student's progress in class. Many programming environments now capture complete time-stamped records of students' actions during programming. In this work, we leverage this rich, fine-grained log data to build a model to predict student course outcomes. From the log data, we extract patterns of behaviors that are predictive of students' success using an approach called differential sequence mining. We evaluate our approach on a dataset from 106 students in a block-based, introductory programming course. The patterns extracted from our approach can predict final programming performance with 79% accuracy using only the first programming assignment, outperforming two baseline methods. In addition, we show that the patterns are interpretable and correspond to concrete, effective -- and ineffective -- novice programming behaviors. We also discuss these patterns and their implications for classroom instruction.

==> SIGCSE'21 - Performance Prediction - ArXiv 2/sections/conclusion.tex <==
% With increasing interests in predicting students’ performance in introductory computing courses, machine learning techniques are largely adopted by researchers to investigate early and precise predictors of students’ performance. However, existing approaches are mostly limited to static students' features but lack investigation with students’ patterns from programming log data that is fine-grained, or are hard to be interpreted for easy understanding. Thus, there is a need for approaches that are interpretable and log data-driven. To fulfill the need, we design an approach that generate interpretable and predictive patterns from students’ log data. We assess our approach with students’ log data from an introductory course which employs a block-based IDE in the classroom. The generated patterns can predict final programming performance with $79\%$ accuracy within just the first exercise. Also, we show that the patterns correspond to concrete novice programming behaviors, such as abstraction, debugging, testing before using. And we provide additional insights into how these patterns manifest in classroom. Since our model is evaluated in the block-based programming context and our results show log data can effectively be used for prediction and reflect students’ programming behavior, we propose to verify our work in other classrooms or contexts in the future. 
Overall, the \textbf{contributions} of this work are: (a) we adapt a sequence mining method to programming log data; (b) we demonstrate that our data-driven approach can generate patterns that predict students final course performance with accuracy $\sim$79\%, using log data from just the first assignment; (c) we show how patterns extracted by our approach can inform our understanding of students' programming behavior.

There are two primary limitations in this study: 1) The specific patterns we find are not all generalizable, with some specific to Snap. However, while the individual patterns may not generalize to all contexts, the method should generalize to any context where we have event-level data with ProgSnap2 format. The patterns and our model are evaluated by hold-out 10-fold cross validation, which suggests we will achieve similar results on a new dataset from a similar population. Additionally, many of these events are general across both block-based and textual programming environments. 2) The data does not come from the typical CS class (only 5 programming assignments), and we do not use any external measures (e.g. quizzes). Future work is needed to evaluate the approach in more classroom contexts, including more traditional CS1 courses. %What is important is programming log data tells us more than static data, and setting the expectations appropriately about what they are going to get.



==> SIGCSE'21 - Performance Prediction - ArXiv 2/sections/exp.tex <==
%In this section we investigate our RQs: \textbf{RQ1:} How do students' patterns of programming predict their final performance in a course, and how early can we make this prediction? \textbf{RQ2:} How do the patterns generated by such an approach inform our understanding of what student programming behaviors suggest that they will struggle in the course? \textbf{RQ3:} Does adding environment-specific contextual information to patterns improve the predictive accuracy and interpretability of the model?

\subsection{Population and Data}
\label{subsec:population}
% Describe your dataset and the students: refer to https://csedresearch.org/reporting-activities/

We use data from an introduction to computing course for non-majors at a large, public university in the Eastern United States. The instructors were not part of the research team. The data was collected across two semesters, Spring 2017 and Fall 2017, with a total of 106 students. In both semesters, students worked on the same 5 programming exercises (A1-A5) in a block-based programming environment called Snap. %where A1, A3, and A5 are lab assignments while the rests are homeworks. %Blocks in Snap are selected from a palette at the side of the screen, which is divided into categories. Students can only open one category at one time. 
We did not have access to students' demographic information or prior experience, but the course was designed for novices. The programming part of the course was taught in labs led by undergraduate TAs. As students worked, the programming environment automatically logged each action a student took (e.g. adding a code block, running code), including complete snapshots of students' code, allowing researchers to recreate a students' programming process.

Rather than using in-class grades which are made by undergraduate TAs (which vary year-to-year), we regraded the exercises with a similar set of rubrics, using the final snapshot of each student’s program, based on the exercise's objectives. We treat the average of students’ grades on these exercises as a measure of their programming performance over the whole course, with the grade of each exercise scaled to (0, 1). We used a median split to divide the students into 54 high performers and 52 low performers, based on a median grade of 0.84. As noted in prior work, a median split is appropriate for evaluating the performance of the classification models as well as identifying the patterns that can significantly differentiate high and low performers \cite{ames1988achievement, ghantasala2013median}. This aligns with our goal of identifying students who will perform worse than others and might benefit from prioritized help (not only students `at-risk' of failing). Our log data is in a well-defined data sharing format, ProgSnap2 \cite{price2020iticse}, and we use it to extract patterns by CDSM. In this study, our data consists of $\sim$530 sequences and $\sim$500 events per sequence.  

%The course is a computer literacy course that aims at non-majors with 3 primary units: programming in Snap, HTML, and spreadsheets. We primarily interested in programming ability of students. However, the in-class assessments cover a number of other course topics which are not related to programming. Therefore, we use students’ programming assignments from the first unit, and treat the average of students’ performance on these exercises as a measure of their programming performance (high vs. low performance) over the whole course. %Rather than using in-class grades which are made by undergraduate TAs (which vary year-to-year), we regrade the assignments using similar rubrics using the final snapshot of each student’s program, based on the assignment objectives. In each semester, students are given 5 programming assignments: PolygonMaker (A-PM), Squiral (A-SQ), GuessGame1 (A-GG1), GuessGame2 (A-GG2), and GuessGame3 (A-GG3). A-PM, A-GG1, and A-GG3 are in-lab assignments, while A-SQ and A-GG2 are homework assignments. The knowledge of specific programming concepts in the 5 assignments are accumulated. We defined each assignment into a set of 5-6 objectives, where each objective represents a rubric item. For each objective, we give point 0, 1 or 2 if a student did not attempt this objective, just attempted it, or completed it correctly, respectively. We then calculate the sum of all objectives (total grade) and normalize it for each exercise within the 0.0-1.0 scale. The Final course grade is calculated by averaging normalized grades of each exercise a student has submitted in the whole semester. Specifically, students whose final grades are at least the median grade are labeled as high performers ($n=54$) while the rest are labeled as low performers ($n=52$). We select the median (0.95) as the split point since it is appropriate for evaluating the performance of the classification models as well as identifying the patterns that can significantly differentiate high and low performers, as suggested by previous studies \cite{ames1988achievement, ghantasala2013median, spence1983achievement}.

%The required knowledge of programming concepts in the five assignments are designed by experts. In particular, A-PM requires the use of custom blocks, functions, drawing, and loops. In addition to what A-PM requires, A-SQ requires the use of variables, and nested loops. A-GG1 used the same but additionally requires interaction with users, and use of if conditions. A-GG2 is the second level of A-GG1, and additionally requires the use of lists. Finally, A-GG3 is the third level of A-GG1, where it uses all concepts in A-GG2, but is more challenging and requires nested if conditions. 



\vspace{-0.1 in}
\subsection{RQ1: Performance Prediction}
\label{subsec:prediction}
%on how early the model can make reliable predictions, since early feedback allows the instructor to adjust the lesson plan accordingly where both the high and low performers can benefit from.

Since RQ1 asks how early we can predict students' grades, we performed 5 separate prediction trials (M1-M5). For a given trial, $M_i$, we only used data from assignments $A_1$ through $A_i$. All trials predicted students' final performance. We extracted patterns from each assignment individually, as completing each assignment requires different programming knowledge, and students’ behavior can change as the course progresses. %Therefore, we propose a feature stacking approach which can normalize and merge the patterns selected by the CDSM from all the milestones released until upon a specific time (e.g. all the assignments released and graded before midterm), as well as a set of prediction models where each one is optimized towards processing the patterns gathered from a certain time step of the course. Specifically, as introduced in Section \ref{subsec:population}, the dataset we consider contains five assignments -- A-PM, A-SQ, A-GG1, A-GG2 and A-GG3, where each one is treated as a milestone of the course. Hence, 5 prediction models are trained to predict students’ final performance, respectively, given each assignment and the previous ones. For instance, model 1 (M1) only takes as input A-PM, model 2 (M2) takes as input A-PM and A-SQ, model 3 (M3) takes as input A-PM, A-SQ and A-GG1 etc.\footnote{To simplify presentation, Model 4 (M4) and model 5 (M5) are omitted from this example but they follow the same mechanism, where M4 takes as input A-PM, A-SQ, A-GG1 and A-GG2, and M5 takes as input all five assignments.}
We adopted a \textit{feature stacking} approach, which combines features across assignments to construct a meta feature table. %Specifically, we first extract patterns using the CDSM on a single assignment basis. Before training each prediction model, patterns from corresponding assignments are stacked together to construct a meta feature table which is then used as training inputs.
%For example, %while training M2, 
%assume we extract patterns $\{P_{1}^{(1)}, P_{1}^{(2)}\}$ from exercise A1 and pattern $\{P_{2}^{(1)}\}$ from exercise A2. Then the set of patterns $\{P_{1}^{(1)}$, $P_{1}^{(2)}$, $P_{2}^{(1)}\}$ will be used in M2 to predict students' final performance after the second assignment. 
We used an Ada-boost classifier and validated it with a modified hold-out 10-fold cross validation, where 8 sets are used for training, 1 set for testing while the remaining one is discarded. %All hyperparameters used in the classifier were tuned during training using the validation set.

Our CDSM approach largely uses generic events which exist in any IDE. We wanted to explore how adding IDE-specific context might improve the CDSM approach. We therefore evaluated 2 variants of the Event Categorization approach detailed in Section \ref{subsec: event_categorization}: the \textit{general} approach, which only captures generic event information (as described earlier), and the \textit{contextual} approach, which also captures a small amount of Snap-specific contextual information.  Specifically, contextual events append a suffix to each action with the name of currently opened block category in Snap (describing what type of blocks a student can add). For example, when an EDIT-INS-pen action is recorded, it means that a student is programming in Snap with \textit{Pen} category opened. Consequently, two explanation levels -- \textit{general} and \textit{contextual} -- of event categorization techniques can be combined with the CDSM to produce patterns with different levels of explainability, which are denoted as \textbf{CDSM-G} and \textbf{CDSM-C} respectively.


%\subsubsection{Baselines}

We employ two baselines: 1) \textit{Majority}: using the majority label of performers as predicted label. %Since we performed a median split on students' overall grade, in our dataset, 54 students are labeled as high performers while the remaining 52 as low performers. Thus, the Majority model always predicts a student as a high performer. 
2) \textit{Expert Rule}: using students' grades on prior exercises (e.g. grades of A1 and A2 for trial M3), as well as 5 expert-authored process data features: \textit{Block Deletions} (number of blocks deleted), \textit{Block Moves} (number of blocks moved), \textit{Code Runs} (number of program run events), \textit{Time} (the total minutes spent on programming exercises), and \textit{Meaningful Nodes} (the total number of loops, conditionals, and custom blocks made by students in their code). Each of these features has been found to correlate with student performance in previous research (e.g. \cite{carter2015towards, emerson2019predicting, hsu2003hybrid, leinonen2017comparison}). Note that Snap does not have compile events, so we could not use compilation error metrics as a baseline. We also employed an Ada-boost classifier with the features from the \textit{Expert Rule} baseline, using the same procedure to tune hyperparameters as our approach.    %The details of the features are presented in the followings:
% \begin{enumerate}
%     \item \textit{Block Deletion}: The number of blocks deleted logged by system over a course. 
%     \item \textit{Block Moves}: The number of blocks moved logged by system over a course.
%     \item \textit{Run Code}: The number of students running programs logged by system over a course.
%     \item \textit{Time}: The total time (minutes) spent by a student on programming exercises over a course.
%     \item \textit{Meaningful Nodes}: The total number of meaningful nodes in logged programming codes over a course, including loops, conditions (e.g. If-Else), and custom blocks made by students.
% \end{enumerate}

%The baseline \textit{Count} will also be a classification with the 5 approaches and validated by a modified hold-out 10-fold cross validation, where 8 sets is used for training, 1 set is designated as test set and the remaining set is discarded.\footnote{ Note that nested cross validation cannot be applied here since no parameters need to be tuned with the \textit{Count} baseline, to keep consistency we evaluate the performance of this approach following this tweaked 10-fold cross validation mechanism.}

\vspace{-0.1 in}
\subsection{RQ2: Pattern Interpretation}

We investigated a meaningful subset of the patterns generated by the CDSM approach to evaluate whether they corresponded to meaningful student behaviors. 
%Our CDSM approach can generate a great amount of patterns at a time. %it is hard to tell which are meaningful in terms of students’ specific programming behavior at first glance%(e.g. the patterns that can be analyzed or interpreted by further qualitative research). 
To investigate these patterns, we recorded all patterns extracted from CDSM with their corresponding assignment name and performance group. Then for each pattern, we calculated: 1) portions (i.e. $Perc\_High$, $Perc\_Low$) of \textit{all} students who have the pattern among high and low performers respectively; 2) the difference (\textit{Diff}) between $Perc\_High$ and $Perc\_Low$; 3) the Odds Ratio (OR) which shows how much more/less likely students who do the pattern are to be low performers. We sorted the patterns by their \textit{Diff} in descending order. Statistically, the higher \textit{Diff} implies the more likely a pattern happens in a specific group. We selected a set of the top $15\%$ of patterns from both performance groups. This helped us identify the most frequent patterns and avoid missing important patterns. For each pattern in the set, 3 researchers replayed the logged actions of individual students who performed the pattern to explore how and in what context the pattern happened during students’ programming process. Each researcher summarized their understanding of the pattern independently, then they discussed their interpretations with 2 criteria: 1) what are students doing within the pattern? 2) how might the pattern be indicative of student performance? If all researchers noted that a pattern reflected was indicative of high- or low-performing students, this suggested that the pattern may be meaningful and interpretable. 



%\subsection{RQ3: Context-Specific Information}
%To examine our RQ3, we propose another event categorization technique (called \textit{contextual}) by building on top of the one introduced in Section \ref{subsec: event_categorization} (which is referred to as \textit{general} in the rest of the paper). Specifically, we append a suffix to each action with the name of currently opened category in the log events. For example, when a EDIT-INS-pen action is recorded, it means that a student is programming in Snap with \textit{Pen} category opened, she might drag either a block (e.g. `pen down’) from \textit{Pen} category or an existing block (e.g. `move’) which may belong to another category from her code. We use the currently opened category as it reflects current programming circumstances that students are working in. Consequently, two explanation levels -- \textit{general} and \textit{contextual} -- of event categorization techniques can be combined with the CDSM to produce patterns with different levels of explainability, which are denoted as \textbf{CDSM-G} and \textbf{CDSM-C} respectively.

%Then, each prediction model is trained on \textit{cdsm-general} and \textit{cdsm-contextual} separately using hold-out 10-fold cross validation. Specifically, we randomly split students into 10 sets within the high and low performance student groups respectively. Then in each training epoch, 8 sets are selected as training sets, 1 set is used as validation set and the remaining set is designated as test set. We don't employ fully nested cross validation because training process of that takes a long time, and our approach will only make the model worse, so our results are pessimistic not optimistic. The features are selected using only the training sets, and we get different features for each round of cross validation. To fit classifiers on each training set, we first employ the CDSM algorithm\footnote{either CDSM-G or CDSM-C} on the log data of the students from the training set. The thresholds in the CDSM are set as follows -- 0 for maximum gap, 6 for maximum length, 0.5 for minimum percentile support, and $\alpha=0.05$ for $\chi^2$ and t-test. By selecting 0.5 as the minimum percentile support means we look into patterns which can be identified from at least 50\% of students in each group. These thresholds are also employed by previous pattern mining study for comparing learning behaviors except maximum gap, e.g. Kinnebrew et al. employed 1 as the maximum gap to avoid noise \cite{kinnebrew2013contextualized}. However, in our study, permitting gaps among actions can ignore some information that might be important (e.g. a quick switch between two block categories), and we want to investigate transactions among actions. Thus, we use 0 as the maximum gap, which means any consecutive transactions among different types of actions will be catched. Notably, patterns are extracted on a per assignment basis. To construct the feature table for each prediction case, we apply the \textit{feature stacking} approach introduced above. Finally, to thoroughly evaluate the performance and generalizability of the CDSM algorithm, we train and test using 5 classification algorithms for each prediction model -- Ada-boost (Ada), Gradient-boost (Grad), Random Forest (RF), support vector machine (SVM), and k-nearest neighbors (KNN). 








==> SIGCSE'21 - Performance Prediction - ArXiv 2/sections/intro.tex <==


%Introductory computing classes have notoriously high failure rates of around 30\% \cite{bennedsen2019failure, watson2014failure}. This statistic is often cited to justify the need for more student support. %though it also suggests that there are specific students who would benefit most from this support. 
%For example, some students might be stuck at an early stage of studying programming and need help, and the risk of failing the course will be raised rapidly if they do not get timely support. 
Many students struggle during introductory programming courses, failing classes \cite{bennedsen2019failure, watson2014failure} or dropping out of CS programs \cite{chen2013stem}. One-on-one instructor guidance is one of the most effective ways to help struggling students \cite{bloom19842}, but instructors have limited time to spend with individuals. What if an instructor could know after a student's first programming assignment whether the student will be a low performer in the course? This would allow an instructor to focus their finite resources on helping the students who stand to benefit most from them. It would also allow researchers to personalize  automated help (e.g. hints and feedback \cite{price2017hint, rivers2013automatic}), to offer higher levels of scaffolding only to students who need it.

%Researchers in many domains have extracted student-related features to address this challenge. 
Prior work has constructed machine learning approaches to predict students' performance in a given course based on \textit{static} and \textit{general} factors, such as grades in their previous courses, majors, and demographic factors \cite{elgamal2013educational, hu2019reliable}. These models have achieved some predictive success. However, few models use factors specific to Computer Science, such as students' programming behavior. Additionally, by focusing on static features (e.g. GPA, demographics), these models might suggest that a student's potential to succeed is fixed, rather than a dynamic product of their in-class effort. There is also a need for more \textit{interpretable} predictive models, which can tell us not only \textit{whether} a student will succeed, but also offer insight into \textit{why}, with implications for pedagogy.

Many programming environments capture rich log data as students work, including detailed, sequential records of students' interactions with the environment \cite{hosseini2014exploring, piech2015deep, price2017isnap}. Prior work has shown that analysis of this \textit{process data} can lead to more accurate predictions of student performance than static measures (e.g. assignment grades) \cite{blikstein2014, hadwin2007examining, piech2015deep}. Log data also captures the same information that an instructor might observe when watching a student program, suggesting potential for data-mined patterns to be interpretable by instructors. Many existing approaches for predicting students' final performance with process data use expert-defined metrics, for example based on students' patterns of compiler errors \cite{becker2016new,carter2015towards}). However, these metrics require extensive researcher expertise to author manually, and are only weakly predictive of student outcomes \cite{price2020iticse}.


To address these limitations, we propose a novel, \textit{data-driven} approach for predicting student course outcomes based on their \textit{process data} (i.e. interactions with the programming environment). We extract patterns of students’ actions from their log data on \textit{early assignments}, which are predictive of their \textit{final} performance in a course. We evaluate our approach in a block-based programming course, finding that some of these patterns correspond to meaningful novice programming behaviors and present case studies of how they manifested in individual students. Specifically, we investigate two research questions: 

\textbf{RQ1:} How do students' patterns of programming predict their final performance in a course, and how early can we make this prediction? 

\textbf{RQ2:} How do the patterns generated by such an approach inform our understanding of how students struggle and learn to program? 
%\textbf{RQ3:} Does adding environment-specific contextual information to students' actions improve the predictive accuracy of the patterns?


%In this work, we identify patterns of students' interactions with the programming environment that are disproportionately common in low- or high-performing students. We show that, when used in a prediction model, these patterns predict students' performance with $\sim$79\% accuracy , 25\% better than chance, and 23\% better than expert baseline using only static features. We also attempt to interpret the patterns to understand why they are predictive of students' success. We compare these findings to prior computing education research on effective and ineffective novice programming patterns. We find abstraction and debugging behaviors are associated with success/failure, which agrees with prior work, and we propose some new possible behaviors that merit further investigation. 


Our \textbf{contributions} are three-fold: (a) we present a sequence mining method for programming log data, based on effective approaches in other domains; (b) we demonstrate that our data-driven approach can generate patterns that predict students final course performance with $\sim$79\% accuracy, using log data from just the first assignment; (c) we show how patterns extracted by our approach can inform our understanding of students' programming behavior. 


==> SIGCSE'21 - Performance Prediction - ArXiv 2/sections/literature.tex <==
%\subsection{Models to Predict Programming Performance}

Many approaches have been proposed for making early predictions of student outcomes in CS courses. These approaches generally consist of two steps: 1) extracting relevant features and 2) training a machine learning model to predict outcomes. Here we focus on the \textit{feature extraction} step. These features can be generally categorized into four types:


\textbf{Background Features}: These are static features about a student or their history before entering the course, such as demographics, GPA, and prior courses taken \cite{elgamal2013educational, hu2019reliable}. For example, ElGamal et al. predict students' programming performance based on their demographics such as gender and prior experience \cite{elgamal2013educational}. However, these approaches require that instructors collect this data, which is not always done. Additionally, these features only reflect a student's background, and not their effort in the course, and their predictions may therefore promote an unproductive \textit{fixed mindset}, rather than a \textit{growth mindset} for instructors who use them \cite{murphy2008dangers}.


\textbf{Grade Features}: These features use students' grades on prior assignments \textit{within a given course} to predict later course outcomes \cite{castro2017evaluating, romero2008data}. For example, Castro-Wunsch et al. counted passed and failed assignments as predictors of struggling students \cite{castro2017evaluating}. These features do capture students' in-course performance and effort; however, student grades only describe a students' final product, and lose relevant information about \textit{how} the student created it.


\textbf{Expert-authored features derived from Process Data}: These features are \textit{defined by experts} and extracted from students' \textit{process data} as they work, e.g. on programming assignments \cite{ahadi2015exploring, castro2017evaluating, emerson2019predicting} or clicker questions \cite{liao2019robust, porter2014predicting}. They might be simple counts of student actions (e.g. steps taken \cite{ahadi2015exploring} or submissions \cite{emerson2019predicting}), or more complex metrics derived from student action sequences. For example, error metrics, such as the Error Quotient \cite{jadud2006methods}, NPSM \cite{carter2015towards, carter2017using} and others \cite{watson2013predicting, becker2016new} quantify the extent to which students struggle with error metrics based on a sequence of their compilation and other behaviors (e.g. create break points \cite{carter2015towards}). However, these features require careful expert authoring, based on observations of student behavior, and as such they may not generalize to new datasets, and can have low predictive accuracy \cite{price2020iticse}.


\textbf{Data-mined features extracted from Process Data}: These features are extracted \textit{automatically} (or semi-automatically) from students' programming process data \cite{wangcomparing}, \textit{discovering} behaviors that might be predictive of student success, beyond what experts have identified. For example, Blikstein, Piech, et al. \cite{piech2012modeling, blikstein2014} used learning analytics approaches to cluster students' problem-solving trajectories on programming assignments and found these clusters to be predictive of students' final grades, moreso than midterm grades. Mao et al. used temporal pattern mining approaches to extract features from sequences of programming snapshots \cite{mao2020time}. These models showed strong predictive success, though they predicted performance on a \textit{single assignment}, rather than across the semester, as in this work. From a theoretical perspective, Grover et al.'s hypothesis-driven framework for learning analytics \cite{grover2017framework} argues that students' fine-grained interactions can serve as meaningful evidence of specific competencies, arguing that ``students’ actions need to be detected and measured as students work.'' They demonstrate how patterns mined from student process data can also be used to inform our understanding of how students express those competencies, though they stop short of using these mined patterns in their assessment models.

In this work, we compare data-mined process data features to a baseline model that uses grade and expert-authored features to determine whether data-driven features improve our ability to predict student outcomes. 

\iffalse

Students' problem solving actions within an integrated development environment (IDE) can serve as an important indicator of their knowledge \cite{molnar2018efficacy}. Previous work has extracted predictive metrics from patterns of actions in an IDE, such as \textit{error metrics} \cite{jadud2006methods, watson2013predicting, becker2016new}, which focus on patters of students' compiler errors. For example, Jadud et al., found that the Error Quotient metric correlated weakly with students' course grades \cite{jadud2006methods}. %Also, Shute et al., according to the stealth assessment approach, showed that they can assess students' knowledge from log data of a well-designed game \cite{shute2013stealth}. 
However, their approaches cannot be applied to many block-based programming environments that do not contain compiler errors and show weak prediction effects of student outcomes \cite{price2020iticse}. In addition, previous research has used a variety of data-driven approaches such as unsupervised techniques, learning analytics, and clustering to predict students performance in a course by extracting programming patterns and program state transitions \cite{baker2014educational, berland2013using,piech2012modeling}. For example, within each assignment, Piech et al., predict whether students will struggle on course materials, by using distance metrics that measure dissimilarity between researcher-selected code snapshots \cite{piech2012modeling}. These approaches, however, focus on tracking snapshot changes from either program states or several ``high-level milestones'' \cite{piech2012modeling} of assignments that each snapshot is pre-selected by researchers, which lack insights into precise students' actions that are more fine-grained. To fill in this gap, in this work, we explored using students' action transitions within a program, which is a more fine-grained data, to predict students' success. 

Previous studies have predicted students' performance in terms of final grades, dropout, etc \cite{hu2019reliable, mao2019one, sahebi2016tensor}. Researchers have been using the students' longitudinal grades to predict their performance across future courses, using regression approaches \cite{elbadrawy2016predicting} or deep learning models \cite{kim2018gritnet, hu2019reliable}. Sahebi et al. proposed a matrix factorization method that can predict student grades from MOOC data \cite{sahebi2016tensor}. Su et al. used students’ past answers to exercises to predict their performance on future exercises using deep neural networks \cite{su2018exercise}. Similarly to our approach, Mao et al. used a recent temporal pattern mining to predict whether a student would succeed or not on a single assignment \cite{mao2019one}, which is different from our goal. However, it is difficult to interpret these models to inform our understanding of learning because typically inspectable students models are quite complex and can be costly to implement \cite{bull2002helping}, and understanding the models requires sufficient knowledge in computer science field such as knowledge tracing and deep learning \cite{mao2019one, piech2015deep}. To make predictive models effective in real classrooms, instructors, who are the ones that provide direct feedback to students, should be able to process and understand the outputs of such prediction models. As a result, there is a crucial need to design and develop interpretable prediction models to help instructors understand students behavior and provide appropriate support to students. Moreover, the previous approaches rely on static information in addition to log data, such as students’ demographics information or previous course grades, in order to make accurate predictions. However, only students’ log data is sufficient for our approach, which could be unfair to select those approaches as baselines in our model evaluation.

% \subsection{Informative Novice Programming Behavior}

% In programming languages, like Scratch, previous studies indicated some bad programming practices that students adopt when learning in these environments \cite{moreno2014automatic}. For example, Moreno-León et al., noted that using non-significant names for sprites and duplicate scripts are bad programming habits in Scratch \cite{moreno2014automatic}, and Aivaloglou et al., found that dead code is another bad habit \cite{aivaloglou2016kids}. In addition, Techapalokul identifies that broad variable scope and uncommunicative naming for objects are the most frequent code smells for bad programs in Scratch \cite{techapalokul2017sniffing}. Aside from exploring bad habits, Dong et al., manually investigated students' actions during programming to define tinkering behavior, which can help in designing better interventions to improve students learning in block-based programming environments \cite{dong2019defining}. They found that moving blocks back-and-forth, or inserting and removing blocks indecisively is a main theme of tinkering indicating a behavior of uncertainty or hesitation, which is also known as a negative behavior of novice programmers \cite{dong2019defining, perkins1986conditions}. Furthermore, researchers noticed that contextual factors can affect students' programming practices. For example, Carter et al., found that highly performing students receive more help from their instructors \cite{carter2015towards}, while Price at al., found that low performing students submit more attempts than high performers \cite{price2020aied}. However, we still do not know empirically whether these observed `bad behaviors’ are really associated with ineffective programming. It’s important to see evidence of these in log data. 


% Not only does investigating students' actions during programming reveal bad and good programming habits, it also reveals the development of Computational Thinking (CT) of students. Why should we expect evidence of student success to show up in log data? Two really important characteristics of programming learning, abstraction and debugging, should show up in programming behavior in these ways: 1) Abstraction, which represents students' captures of essential aspects and reducing complexity of their programs \cite{haberman2004high, mostrom2008concrete}, is associate with students’ ability with program construction \cite{vainio2007factors}. Students who lack abstraction perform to be confused with high-level programming concepts \cite{vainio2007factors, ye1996expert}. Vainio et al. found that students lacking abstraction would encounter difficulties with tracing variables and usage of loops \cite{vainio2007factors}. Vainio et al. found that novice programmers are performing worse on functions with C programming language than experts \cite{ye1996expert}. 2) Time spent on debugging a program is associated with students’ evaluation ability on learning materials \cite{bloom1956taxonomy, renumol2009classification}. Leinonen et al. found that struggling students tend to debug programs when encountered with difficulties \cite{leinonen2017comparison}, while Alaqdi et al. found quicker debug are more employed by experienced students \cite{alqadi2017empirical}. Students employ various debugging strategies (e.g. using the debugger) and some ineffective strategies would have specific patterns (e.g. tinkering) \cite{fitzgerald2008debugging}. For instance, Chmiel et al. noticed that novices could debug their programs haphazardly without a plan \cite{chmiel2004debugging}. However, these have rarely ever been operationalized and studied quantitatively. In this work, we identify patterns that actually, empirically differ between high/low performing students and we see if they correspond to these hypotheses.    

%\subsection{Theoretical Framing for Data-driven Inference}

In particular, we build our work on the theoretical framework of Grover et al. \cite{grover2017framework}. It blends hypothesis- and data-driven approaches to offer a richer interpretation of student actions, and provides a combined-analysis concept with both qualitative and computational analysis such as sequence mining. They compare students' action sequences between high and low performers to find common behaviors within each performance group. Also, their framework leverages Evidence Centered Design \cite{mislevy2006implications}, which argues that students' fine-grained interactions with a well-designed task can serve as meaningful evidence of specific competencies. However, there are some key differences between their work and ours: 1) While their goal is a detailed and validated assessment of CT, our goal is to identify low-performing students early-on in a semester, which is a much simpler assessment task. 2) While their approach requires students to use tasks that are specifically designed to elicit good evidence, and a multi-stage analysis (e.g. video traces) of students' behavior, our approach is designed to be classroom-ready, and use existing course assignments with only students' log data. 3) While they use a priori hypotheses to identify meaningful action sequences, we employ a data-driven approach to identify action sequences that can then inform hypotheses. Notably, though Grover et al. do suggest some sample patterns and anti-patterns found in log data, which correspond to behaviors they found in video analysis, they stop short of using these in their assessment. However, in this study, we incorporate patterns into a predictive model, and show that they are in fact highly predictive of students outcomes.

\fi

==> SIGCSE'21 - Performance Prediction - ArXiv 2/sections/method.tex <==
% \begin{figure}[t]
% \includegraphics[scale=0.3]{figures/cdsm.png}
% \centering
% \caption{Graphical Structure of Pattern Mining}
% \label{fig:cdsm}
% \end{figure}

%% Dependent-High, Dependent-Low, Frequent-High, Frequent-Low

% intro
%Our main goal in this study is to extract predictive patterns in fine-grained log data from students' interactions with a block-based programming environment towards their final programming performance. %We focus on these patterns because we hypothesize that they can be interpreted to gain insights into the programming behavior of successful students. In this section, 

We present $\chi^2$ - differential sequence mining (CDSM), a data-driven feature engineering algorithm, designed to identify sequences of events (i.e. patterns) in students' log data that differentiate two groups of students: high-performing (\textbf{HP}) and low-performing (\textbf{LP}) students. Specifically, the method identifies two types of patterns: 1) patterns that occur for \textit{more students} in one group than another (e.g. 30\% of LP students vs. 60\% of HP students), and 2) patterns that occur for students in both groups, but appear \textit{more times} for students in one group than another (e.g. an average 5 times per assignment for HP students vs. 1 time per assignment for LP students). The presence of these patterns can then be used as features in a predictive model. 

CDSM builds on the original differential sequence mining (DSM) approach of Kinnebrew et al. \cite{kinnebrew2013contextualized}. We extend this approach in 3 ways. First, we define an \textit{event categorization} method for extracting discrete, meaningful events from programming process data (Section~\ref{subsec: event_categorization}). We then extend DSM to detect less frequent, but still discriminating patterns using a $\chi^2$ test (Section~\ref{subsec:pattern_mining}). Last, we use feature discretization to improve the performance of the extracted features in a model (Section~\ref{subsec:discretization}).

\subsection{Event Categorization}
\label{subsec: event_categorization}

For each student in class, their log data can be represented as a sequence of discrete events that occurred during programming assignments, along with a label (e.g. high/low performing). The sequence should capture all student interactions with the programming environment (e.g. editing code), as well as other interface actions (e.g. menu clicks). The first challenge for the algorithm is to represent these events with the right level of granularity. For example, if events are too specific (e.g. treating every keystroke as a unique event) it will be difficult to find shared patterns across students, but if they are too general (e.g. one event for all code edits), patterns may not be meaningful.

To address this, we leverage the event categorization scheme of the ProgSnap2 format for programming log data \cite{price2020iticse} to make our approach more generalizable across datasets, as ProgSnap2 is designed to represent students' interactions within a variety of programming environments (e.g. block- and text-based) and educational settings. This allows us to build on established event definitions and makes it straightforward to apply our approach to a growing number of programming datasets using ProgSnap2 format. %ProgSnap2 also allows for datasets to include user-defined event types (prefixed with ``X-'').
Specifically, we used 5 types of events\footnote{We used a subset of ProgSnap2 events relevant to our block-based dataset, but additional events, such as ``Compile'' could be included for other datasets.}: 1) \textbf{EDIT} (File.Edit): The student edits their program. ProgSnap2 also defines several subcategories of EDIT events, and we treat these as distinct events: EDIT-INS: code is inserted into the workspace, EDIT-DEL: code is deleted from the workspace, and EDIT-PST: code is pasted or duplicated into the workspace; 2) \textbf{RUN} (Run.Program): The student runs their program; 3) \textbf{FILE} (File.*): The student performs a file-related action, such as closing, saving, and deleting a file. We collapse these various ProgSnap2 events into a single FILE event type; 4) \textbf{CHAN} (X-ChangeBlockCategory): The student selects a different block category (events prefixed with `X-' are specific to our dataset, described in Section~\ref{subsec:population}); 5) \textbf{VAR} (X-AddVariable): The student creates a new variable.

%ProgSnap2 also allows for datasets to include user-defined event types (prefixed with ``X-''). The dataset we use in this work (detailed in Section~\ref{subsec:population}) comes from the block-based Snap programming environment \cite{Garcia2015}, and defines 2 additional event types:
%Blocks in Snap are selected from a palette at the side of the screen, which is divided into categories (e.g. Motion). 
    
     %using Snap's menu interface.

\vspace{-0.1 in}
\subsection{Pattern Mining}
\label{subsec:pattern_mining}

\begin{figure}[t]
\includegraphics[scale=0.17]{figures/cdsm.png}
\centering
\caption{Schematic of the Pattern Mining Algorithm. %In Layer 1, Sequential Pattern Mining (SPM) and $\chi^2$-test are performed to select patterns that are significantly occurred in high- and low-performance group, respectively. Then the remaining patterns are further classified to associate with the two performance groups in Layer 2.
}
\label{fig:cdsm}
\vspace{-0.2 in}
\end{figure}



After categorizing all events in the trace data, all the actions taken by students in each programming assignment can be formulated as a sequence of events. To simplify the representation of sequences, consecutive actions of the same type are collapsed into a single action in this paper (e.g. EDIT RUN is considered instead of EDIT EDIT RUN). This is useful because it collapses similar patterns into one representation, making it easier to find common behaviors among students. However, this also means we may lose some potentially relevant details in the patterns. This choice is designed to strike a balance between specificity and generality. Then the pattern mining step is devised to identify patterns, from these sequences, which can differentiate programming behaviors between two students groups (i.e. HP and LP )regarding their final performance.\footnote{Certain criteria (e.g. course final grade) can be used to divide students into these two groups. } 

To achieve this, we propose a two-layer pattern mining algorithm as depicted in Figure~\ref{fig:cdsm}. In Layer 1, Sequential Pattern Mining~\cite{agrawal1995mining} is first applied to find frequent patterns (\textbf{FP}s) among all the sequences within each performance group, respectively. Then a $\chi^2$-test is performed to identify two types of patterns -- \textit{frequently} high performance (\textbf{FH}) or low performance (\textbf{FL}) , which contain patterns that \textit{frequently} occurred among HP and LP students respectively. The patterns do not show statistical significance in this layer are assigned to the `Medium' group and transmitted to Layer 2. Specifically, we extract FPs according to 3 factors -- minimum percentile support, maximum gaps and maximum length. Minimum percentile support is the minimum portion of sequences that contains a pattern. Maximum gaps is the maximum number of actions can be skipped when constructing patterns within a sequence. Maximum length refers to the maximum number of actions required to construct a pattern within a sequence. Then, all the patterns whose all three factors meet certain thresholds are selected to be FPs. Next, for each FP, we count the frequency of occurrence (FoC) in the HP and LP groups respectively. $\chi2$-test is employed to investigate whether the FoC of a FP \textit{significantly} correspondeds to any performance groups (i.e. HP or LP). If so, the FP is associated categorized as FH or FL.               

In Layer 2, the instance-support~\cite{lo2008efficient} of each FP in the Medium group is calculated, followed by a $t$-test to label it as a dependent-high (\textbf{DH}) or dependent-low (\textbf{DL}) pattern. Specifically, for each pattern, its instance-supports are calculated across all sequences in HP and LP respectively, which then results in two sets of instance-support (i.e. one set corresponds to HP and the other set corresponds to LP). Then, a $t$-test is used to determine whether one set is \textit{significantly} different from the other. If so, then it implies that the corresponding FP appears more frequently in one performance group than the other, and it is associated with either DH or DL depending on the mean value of instance-supports within each group (we select the group with higher mean value). If the $t$-test does not show significance, then the corresponding FP is determined as non-differential patterns and discarded. 



%We want to explore the whole trend across a semester, and the general patterns students might repeat across different exercises. We care about both transactions among different events and explanation of patterns. Thus, if consecutive events are labeled the same, we only record them once in our sequences. For example, a student whose log events are EDIT-INS EDIT-INS EDIT CHAN CHAN FILE will be recorded as sequence EDIT-INS EDIT CHAN FILE. 

%Our pattern mining procedure is divided into two steps, which identify 4 categories of relevant patterns: High-Only, Low-Only, High-Same, and Low-Same as shown in figure \ref{fig:cdsm}. Patterns which significantly only occur in only one performance group belong to High/Low-Only, while patterns which are frequent in both performance groups but more likely to happen in one group belongs to High/Low-Same.

%Step 1 represents the first layer of our pattern mining structure in figure \ref{fig:cdsm}. We extract patterns for each performance group based on traditional sequence mining approach \cite{agrawal1995mining}, which counts the number of sequences containing the pattern. 
%However, previous work strictly divided patterns into high/low-only groups \cite{kinnebrew2012identifying}, which is unfair for patterns that tend to belong to high/low performers only with a small bias. To avoid this, we applied $\chi^2$ test to the first layer. Specifically, for each pattern, we tabulate the data of the two performing groups and the percentages of students who contain the pattern or not. The null hypothesis is each performing group is independent of the percentage of sequences containing a pattern. We select the patterns that fulfill the null hypothesis and put them into High/Low-Only groups. The rest of the patterns remain in the Same group.   

%Step 2 emphasises deeper insight into each pattern within each student, while the first step takes care of significant patterns happening among students. In Step 2, for each pattern in the Same group, we count frequencies of the pattern happened within each sequence (named \textit{episode frequency}) and apply t-test to check whether the average value of the pattern's episode frequency across all sequences in one group differs significantly across the performing groups \cite{kinnebrew2012identifying}. The patterns which are proved significant will be added into the High/Low-Same group.
\vspace{-0.1 in}
\subsection{Feature Discretization}
\label{subsec:discretization}

As prediction techniques usually require numeric inputs, the patterns we obtained from the pattern mining procedure need to be cast as numerical features. To achieve this, we design a tabular feature representation method. Specifically, we store the FoC of all FPs in the 4 categories in a feature table where each column corresponds to a FP and each row corresponds to a student. %Note that $i\in[1,N]$ and $j\in[1,K]$, where $N$ represents the total number of students and $K$ is the total number of FPs that are in the union of FH, FL, DH and DL. Hence, each cell ($S_j$, $F_i$) represents the frequency of FP $F_i$ occurring in the sequence of the student $S_j$. However, due to the varied length of sequences and patterns, the ranges of FoC across columns can be varied. As a result, a normalization process is necessary as it can improve the performance of the classification model, and 
We use discretization in this work since it has low computational complexity and has generally shown a good performance on classification tasks \cite{frank1999making}. Specifically, for the columns that are associated with FH or FL, all the containing FoCs are discretized into two equal-frequency bins. The cells that are smaller than the median are assigned with 0's, while the others are assigned with 1's. Similarly, for columns belonging to DH and DL groups, all the FoCs are discretized into three equal-frequency bins with values 0, 1, and 2 using 1/3 and 2/3 quantiles. We split them up into 3 bins because the FPs in DH and DL are more common to appear in both student performing groups (i.e. FH and FL) simultaneously.    


% how to differentiate four groups while input into prediction algorithm

% The pattern mining step classifies patterns into four groups -- High-Only (HO), Low-Only (LO), High-Same (HS), and Low-Same (LS). Each pattern within the four groups is used as a feature, which constitutes the inputs to the prediction algorithm. For each student, the episode frequency of each feature is calculated. Finally, a 2-dimensional table is constructed in which rows represent students and columns represent features.

% Since the ranges of values in the 2-dimensional are varied among features, we discretize the features into bins. Considering the differences among "-Only" and "-Same" groups during their constructive process, we discretize the features under High/Low-Only groups into two equal-frequency bins: 0 and 1, and features under High/Low-Same groups into three equal-frequency bins: 0, 1, and 2.   


==> SIGCSE'21 - Performance Prediction - ArXiv 2/sections/result.tex <==


%---------------------------------------------------------

\subsection{RQ1: Performance Prediction}

\begin{figure}[t!]
\includegraphics[scale=0.33]{figures/ada-result2.png}
\centering
\caption{Visualization of Prediction Results by Adaboost. X-Axis: Trial Number; Y-Axis: Prediction Results.%; From Left to Right: Accuracy, Precision, Recall
}
\label{fig:pred-result}
\vspace{-0.2 in}
\end{figure}

The prediction results from Adaboost classification using patterns generated from our approach and 2 baselines are shown in Table~\ref{table:predRes} and visualized in Figure~\ref{fig:pred-result}. Our approach (CDSM-G and -C) performs better with higher accuracy and precision than both baselines among all trials across exercises, except precision on the 5th trial (M5) of CDSM-C. Our approach reaches to 0.792 accuracy within the first exercise. Specifically, using data from only the first exercise, our approach can identify more than $ 80\%$ of students who will end up as low performers, while miss-identifying less than $20\%$ of high-performers as low-performers (CDSM-G). By contrast, the Count baseline (which included students' actual grades on prior assignments) only reached that accuracy on the last trial, with all available data. We also find that CDSM-C has less accuracy and precision than CDSM-G across exercises, which indicates that contextual information did not improve the prediction.

%In this section, we report accuracy, precision, and recall obtained through the nested cross validation process for all prediction models, where the accuracy of the 5 prediction models, training by combinations of different feature engineering methods (e.g. CDSM-G, CDSM-C, \textit{Majority} or \textit{Count}) and classification algorithms (e.g. \textit{Ada}, \textit{Grad}, \textit{RF}, \textit{SVM} or \textit{KNN}), are shown in Table \ref{table:predRes} and Figure \ref{fig:pred-result} visualizes the results from Adaboost.

%The results contains three major observations: 1) Our models performs better than baselines among all assignments; 2) Our models can identify low-performing students early-on in a semester, especially with only the first assignment, which could be caused by the concatenation of features; 3) Patterns that are more general are more predictive than patterns that are more specific to the programming language, while both can be interpretable (see Section 5.2).

%\subsubsection{Model Performance}

%Students’ patterns of programming have a better prediction effect on their final performance than superficial counts. From the Table \ref{tab:accuracy}, it can be observed that in general our models with the two variants of the CDSM (i.e. CDSM-G and CDSM-C) perform better than the two baselines in terms of accuracy. Specifically, the overall accuracy ranges of \textit{Ada}, \textit{Grad}, \textit{RF}, \textit{SVM} and \textit{KNN} range from 0.641 to 0.850, as reported in Table~\ref{tab:accuracy}. %$[0.773, 0.850]$, $[0.747, 0.822]$, $[0.715, 0.791]$, $[0.641, 0.766]$ and $[0.650, 0.735]$ respectively. 
%In contrast, the \textit{Majority} baseline only attains to 0.509 accuracy, while the \textit{Count} baseline results in accuracy ranges from 0.390 to 0.655. %$[0.396, 0.567]$ for \textit{Ada}, $[0.535, 0.655$ for \textit{Grad}, $[0.390, 0.614]$ for \textit{RF}, $[0.493, 0.608]$ for \textit{SVM} and $[0.466, 0.578]$ for \textit{KNN}.
%This indicates our models can effectively and accurately classify students into high- and low-performing groups on all assignments that are released incrementally over time. Notably, our models can predict students’ final programming performance early in the first assignment with accuracy value 0.792, which is helpful for instructors to identify potential low performers at an early stage and adjust their teaching plans accordingly.

%In addition, our models can identify low-performing students within only the first assignment, with precision ranging in $[0.688$, $0.833]$ and recall ranging in $[0.615, 0.846]$. Notably, with Adaboost, using only the first assignment, the CDSM-C can identify more than $ 80\%$ of low performers, while only miss-identifying less than $20\%$ of high-performers as low-performers. Similarly, CDSM-G can identify around $83\%$ of low performers, while only miss-identifying $23\%$ of high-performers as low-performers.      

%\subsubsection{General vs. Context-Specific Models}
%From prediction statistics, CDSM-G performs better than CDSM-X among all assignments, that means patterns that are more general are more predictive than patterns that are more specific to the programming language context. Specifically, the average accuracy of CDSM-G is $0.758\%$ while the average accuracy values of CDSM-X is $0.740\%$, while the accuracy values ranging in $[0.686, 0.850]$ for CDSM-G and $[0.641, 0.803]$ for CDSM-X. 


% Since sequences are stacked and patterns are extracted separately in each case, we train the classifiers separately for each case. The set of hyperparameters is kept the same among models so we can compare our model to the baselines. Each case in each classifier is evaluated by 10-fold cross validation. We report accuracy, precision, and recall from test sets. The prediction results are shown in Figure \ref{fig:pred-result} and Table \ref{table:predRes}. 

% Our results show 3 key information: 1) Beat baselines; 2) Early prediction; 3) Generalizability. And we describe these in the following three paragraphs. 
% \subsubsection{Beat Baselines}
% Students’ patterns of programming have a better prediction effect on their final performance than superficial counts. From the figure and table, we can see that our model on two explanation levels, CDSM-G and CDSM-X, performs better on both accuracy than the two baselines. However, the essence of predicting by majority is super biased, and it cannot recognize low performers in need when high performers are larger. Thus, majority prediction is not robust for researchers in the Computing Education field, especially ones who care more about low performers to offer support.
%  With average $74.9\%$ accuracy, our model performs 25\% better than the baseline using majority, and $23\%$ better than the other baseline using superficial counting features. XXX(Precision and Recall)
% \subsubsection{Early Prediction}
% Our model can predict students’ final performance at an early stage. With students’ patterns only from the first assignment, our prediction accuracy can reach to $79.2\%$.XXX
% \subsubsection{Generalizability}
% The CDSM-X does not perform better than CDSM-G. The average accuracy of CDSM-G is $75.8\%$ while the average accuracy of CDSM-X is $74.0\%$. XXX By comparing the results of two explanation levels of our model, we can see CDSM-X, which is more specific to the programming language, performs no better than CDSM-G, which is more generalizable. This indicates that using patterns which are more specific to programming languages could be not helpful for improving prediction results. 

\vspace{-0.1 in}
\subsection{RQ2: Pattern Interpretation}

%With each pattern in the set selected from the \textit{pattern interpretation} procedure, we determine students who have the pattern and the time when the pattern occur. Then 3 researchers replayed students’ log data to explore how and in what context each pattern happen during students’ programming process. Then each researcher summarizes their understanding of the patterns independently, followed by discussion of their interpretations regarding the patterns to resolve any discrepancies. 
From the researchers' examination of patterns, we note that: 1) Not all of the patterns were very informative. For example, the ``RUN EDIT-ADD'' pattern was more frequent with low performers, but this only indicates that they are more likely to run their code followed by adding blocks, which is a generic behavior to most students. 2) Some of the patterns are highly related (e.g., EDIT-INS CHAN is a subset of EDIT-INS CHAN CHAN) and convey similar information to researchers. We focus on only one pattern from each cluster of similar patterns. Our analysis discovered $\sim15\%$ distinct, meaningful patterns among the 288 we inspected, from more than 1000 total patterns. Here we focus on case studies of 3 examples (shown in Table \ref{table:pattern}), where all researchers agreed on their interpretability and meaningfulness. %In the \textit{Name} column, ``H'' represents high-performers group while “L” represents low-performers group, “G” represents general patterns while “C” represents context-specific of patterns, and the suffix number represents pattern number. For instance, “HG1” means the first general-level pattern selected by researchers is among high performers. The last column reports the Odds Ratio, which is a measure of the effect size, quantifying the ratio of the odds that high performers exhibit a given pattern ($P(Yes)/P(No)$) to the odds that low performers do \cite{bland2000odds}. Also, we recreate the programming process when a pattern occurs in case studies and label the blocks interacted by students with \textit{stage} number to depict the order of interaction (see Figure \ref{fig:examples}). All 4 of our case studies are from assignments A-SQ and A-PM for simplicity, though we found interesting patterns from others as well. A-SQ requires the student to draw a square-shaped spiral with a number of rotations given by a user, and it requires the use of loops, parameter initialization, user interaction, and the use of parameters. A-PM requires students to write code that can draw a regular polygon with a number of sides, the size of each side, and the thickness of the pen, as well as to understand programming concepts about loops. Both assignments require to make code in a custom block, which is how students define procedures in Snap. Snap allows students to program custom procedures under a ``hat block'' (see the top of Figure \ref{fig:studentA}), which can return values.%Below, we provide a general explanation of the four patterns:

%\begin{enumerate}
%\item \textbf{HG1} (SQ): Students create a custom block (possibly with parameters), then add blocks from 2 different categories. The reason why the first EDIT-INS specifically indicates creating a new custom block (procedure), as opposed to adding a new \textit{code block}, is that it is not followed by an EDIT, which always occurs when students ``drop'' a new code block into their workspace. When students are doing HG1, they are not only creating a custom block, but they also adding new code to it from different categories. This suggests that they are creating a custom block before they create the code that will go inside of it. In contrast, students who write code first, and then move it into a newly created custom block, would not have the 2nd and 3rd EDIT-INS events (since their code would already exist). 

%\item \textbf{HX1} (PM): Students change the block palette category to the \textit{motion} category, then create three blocks in a row while in that category. The only blocks a student can create while in the \textit{motion} category are \textit{motion} blocks or blocks representing the inputs (parameter variables) of an existing custom block. This pattern was identified for the PM assignment, which only requires \textit{two motion} blocks to solve. Therefore, students who exhibited this pattern were often using at least one custom block input, along with motion block(s).

%\item \textbf{LG1} (PM): Students add a new piece of code, edit their code, and run it, and then repeat this process. Recall that a given even (e.g. EDIT) can represent multiple instances of the event occurring in a row, so the events in this sequence may represent a duration of editing or running. When students are doing this, it suggests they are running their code frequently after adding blocks. 

%\item \textbf{LG2} (SQ): Students change category, followed by running their codes, then create several custom blocks, a common block, or several parameters.  
%\end{enumerate}

%We find that students are mostly on the right track to accomplish a programming concept (e.g. nested loops) required in SQ and PM assignments, when they are doing HG1 and HX1. And it seems they are doing the patterns with a clear comprehension of knowledge behind the assignments or an abstract workflow of adding blocks. This kind of behavior, in previous study, is described as abstraction, and it exists among experts who are highly skilled in programming languages more frequently than novice programmers \cite{ye1996expert}. In this study, within novice programmers, the frequency that the behavior happens among high performers ($52\%$) is significantly higher than low performers ($32\%$ for HG1 and $29\%$ for HX1).

%We also find that students are running their codes after one or several edits when they are doing LG1. This is indicative of debugging behavior defined by Bloom et al. \cite{bloom1956taxonomy}. Debugging is not necessarily needed among super-fine-grained edits. It is likely to occur when a student has a working program. In this study, we notice that the portion of low performers who have the pattern ($60\%$) are significantly larger than high performers ($37\%$). It verifies the findings made by Price et al. that running codes multiple times after each edit is a characteristic of low performers \cite{price2020aied}. It also supports the findings made by Bloom et al. that debugging behavior is an important feature of students’ ability on learning \cite{bloom1956taxonomy}. 

%For better understanding of our findings, we depict four examples from students’ log data for the patterns described above.  

\begin{figure} [t!]
     \centering
     \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth, height=3cm]{figures/example/A.png}
         \caption{HG1 of Student A. %Stage 1 (EDIT-INS): Create a custom block. Stage 2 (CHAN EDIT-INS): Change to \textit{Control} category and add a repeat block. Stage 3 (EDIT): Configure repeat block. Stage 4 (CHAN EDIT-INS): Change to \textit{Motion} category and add a block.
         }
         \label{fig:studentA}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth, height=3cm]{figures/example/D.png}
         \caption{LG2 of Student C. %Stage 1 (CHAN RUN EDIT-INS): Change to \textit{Pen} category, test pen down block then add it to stage. Stage 2: Change to \textit{Motion} category (CHAN RUN EDIT-INS), test move block then add it to stage.
         }
         %\label{fig:y equals x}
     \end{subfigure}
        
    %  \hfill
    %  \begin{subfigure}[b]{0.23\textwidth}
    %      \centering
    %      \includegraphics[width=\textwidth,height=3cm]{figures/example/B.png}
    %      \caption{Student B. Stage 1 (CHAN-motion EDIT-INS-motion EDIT-motion): With an opened custom block, change to \textit{Motion} category and add a move block. Stage 2 (EDIT-INS-motion EDIT-motion): Add an existing parameter \textit{size}. Stage 3 (EDIT-INS-motion): Add a turn block.}
    %      %\label{fig:studentA}
    %  \end{subfigure}
    % \hfill
     %\newline
     \begin{subfigure}[b]{0.46\textwidth}
         \centering
         \includegraphics[width=\textwidth, height=2.8cm]{figures/example/C.png}
         \caption{LG1 of Student B. %Stage 1 (EDIT-INS EDIT RUN): Move a block back-and-forth and run code twice. Stage 2 (EDIT-INS EDIT RUN): Create a custom block. Stage 3: Cancel the custom block and run code once.
         }
         %\label{fig:y equals x}
     \end{subfigure}
     %\hfill
    %  \newline
    %  \begin{subfigure}[b]{0.23\textwidth}
    %      \centering
    %      \includegraphics[width=\textwidth, height=3cm]{figures/example/D.png}
    %      \caption{Student D. Stage 1 (CHAN RUN EDIT-INS): Change to \textit{Pen} category, test pen down block then add it to stage. Stage 2: Change to \textit{Motion} category (CHAN RUN EDIT-INS), test move block then add it to stage.}
    %      %\label{fig:y equals x}
    %  \end{subfigure}
    %     \caption{Code Stage Examples of Four Students}
    %     \label{fig:examples}
    \caption{Code Construct Examples with Selected Patterns}
    \label{fig:examples}
\vspace{-0.25 in}        
\end{figure}


\subsubsection{Case Study 1: Abstraction}
The HG1 pattern, EDIT-INS CHAN EDIT-INS EDIT CHAN EDIT-INS, was detected for assignment A2 as more common among high performers. In this pattern, students create a custom block (i.e. a procedure), possibly with parameters, then add blocks from two different categories. The reason why the first EDIT-INS specifically indicates creating a new custom block (procedure), as opposed to adding a new \textit{code block}, is that it is not followed by an EDIT, which always occurs when students ``drop'' a new code block into their workspace (i.e. stage). %When students are doing HG1, they are not only creating a custom block, but they also adding new code to it from different categories. 
HG1 also suggests that students are creating a custom block before they create the code that will go inside of it, as students who move existing code into a newly created custom block would not have the second and third EDIT-INS events. While this pattern may seem overly-specific to one programming environment and its logging approach, CDSM's data-driven approach allows it discover similar niche patterns from other log data too.

Student A is a high performer who shows pattern HG1 in A2. %SQ requires the student to draw a square-shaped spiral with a number of rotations given by a user, and it requires the use of loops, parameter initialization, user interaction, and the use of parameters.
Figure \ref{fig:examples} shows the code construct that occurred during pattern HG1 for Student A over 10 seconds. It mainly consists of 4 stages of code changes: 1) EDIT-INS: Create a custom block and a variable named ``number of rotations''; 2) CHAN EDIT-INS: Change to the \textit{Control} category and add a ``repeat'' block with default parameter 10 into stage; 3) EDIT: Configure the ``repeat'' block by updating the parameter to 4; 4) CHAN EDIT-INS: Change to \textit{Motion} category and add a ``move'' block. In this study, the frequency that this behavior happens among high performers is much higher than low performers ($52\%$ vs $31\%$). This could indicate that students with HG1 understood the importance of custom blocks (i.e procedures), and seemed to have a plan for what to do in that block by adding two new blocks right after.

Students who demonstrated HG1 started by defining a procedure, before adding code, suggesting a more-top down design of their program, or at least more familiarity with how to create procedures. Prior studies related such observations to students' abstraction behavior \cite{ye1996expert, wing2006computational}, as procedures allow programmers decompose problems and hide unneeded implementation details. %Since creating procedures is an important element of abstraction, we discuss how students' observed behavior may evidence their computational thinking ability. 

%We can see that student A was creating nested repeat blocks and moving the sprite inside the look within a short time range. This can be seen as an abstraction behavior of high performers %with two points: 1) Creating nested loops is important since it’s a part of key concepts in SQ assignment. Student A not only creates a nested loop, but edits the inputs of the nested loop correctly. 2) 
%Student A started with creating a custom block, then added one block of one type and adds one block of another type. If students do not have a plan in mind, they may not create a custom block to begin with, instead they would start their code with adding blocks haphazardly and drag existing code into a custom block later. These indicate that student A understood the importance of procedures with employing custom blocks, and seemed to have a plan for what to do in that block with adding 2 new blocks right after, % has a good comprehension of programming aspects of SQ and is familiar with Snap environment, 
%which always be related with abstraction behavior \cite{bloom1956taxonomy}.

%There could be different ways HG1 occurs. For instance, students create a custom block, then add one ``pen down'' block from \textit{Pen} category and one ``move'' block from \textit{Motion} category to the custom block. Compared to student A, this is imperfect for interpretation since it’s not clearly related with programming concepts of A-SQ. However, such circumstances are still strongly correlated with abstractions. It is because whenever students perform pattern HG1, they start with a custom block followed by adding blocks instantly, which can show they have a well comprehension on programming concepts (e.g. custom block) and a plan, which is deemed as an important feature of abstraction by Bloom et al. \cite{bloom1956taxonomy}. 

% \subsubsection{Case Study 2: Abstraction}
% The HC1 pattern was detected for A-PM as more common among high performers. Students change the block palette category to the \textit{motion} category, then create three blocks in a row while in that category. In Snap, the only blocks a student can create while in the \textit{motion} category are \textit{motion} blocks or blocks representing the inputs (parameter variables) of an existing custom block. This pattern was identified for the PM assignment, which only requires \textit{two motion} blocks to solve. Therefore, students who exhibited this pattern were often using at least one custom block input, along with motion block(s).

% Student B is a high performer who performs pattern HC1 in A-PM assignment. %A-PM requires students to write code that can draw a regular polygon with a number of sides, the size of each side, and the thickness of the pen, as well as to understand programming concepts about loops.
% Figure \ref{fig:examples} shows code stages captured by B’s changes on his code during the 12s with HC1. With a custom block already created, student B changed the working category to \textit{Motion}, added a ``move'' block, added an existing parameter named ``size'', then added a ``turn'' block. We notice that student B was writing codes for drawing sides of a polygon with parameters. The parameter added in B’s code represents the length of each side of a polygon. Similar to student A, student B was adding blocks constantly and sequentially. This can indicate our pattern mining picked up a specific code pattern that is part of the correct solution, and students who performed worse in the course often failed to do this, with the frequency that the behavior happens among high performers is much higher than low performers ($52\%$ vs $29\%$).
% %One thing is that B kept adding blocks without removing, running his code, or switching categories. The other is that B added a repeat block followed by a move and turn block, unlike other unordered behavior such as creating some blocks then dragging them into a repeat block. These suggest that student B is confident and familiar with the programming environment, and has a clear coding structure in mind on how to finish the assignment. Therefore, under this circumstance, the pattern HC1 can also be seemed as a reflection of abstraction.

% However, pattern HC1 does not have a corresponding significant pattern in general level (e.g. CHAN EDIT-INS EDIT EDIT-INS EDIT EDIT-INS). This may occur because: 1) The pattern is category specific, where the inputs need to be embedded into a \textit{motion} block; or 2) In A-PM assignment, one critical part of the code solution for drawing polygons is two consecutive blocks (move and turn) in the \textit{Motion} category. Recall that there are no other requisite categories for adding at least two consecutive blocks or parameters. This suggests the potential advantages of using a context-specific pattern that related with possible solutions of an assignment. %This indicates that our algorithm can catch critical patterns in granular level, without getting patterns stochastically.

% Overall, we found that patterns HG1 and HC1 related to how students used custom blocks, and block inputs. Since creating procedures is an important element of abstraction, we discuss how students' observed behavior may evidence their computational thinking ability.


\subsubsection{Case Study 2: Debugging}

The LG1 pattern, EDIT-INS EDIT RUN EDIT-INS EDIT RUN, was detected for assignment A1 as more common among low performers than high performers (60\% vs 37\%). In this pattern, students repeatedly add a new piece of code, then edit their code and run it. Recall that a given event (e.g. EDIT) can represent multiple instances of a type of event occurring in a row, so the events in this sequence may represent a duration of editing or running. Student B is a low performer who has the pattern LG1 in the A1 exercise. Figure \ref{fig:examples} shows the code construct captured among student B’s changes on their code within 14 seconds when they are doing LG1. It mainly contains 3 stages: 1) EDIT-INS EDIT RUN: Move a block back-and-forth by grabbing one existing custom block ``Make a Polygon of $\#$ Size $\#$ Sides $\#$ Thickness [sic]'' and snapping it back to the stage. The student then runs code twice but nothing is drawn because of missing parameters inside the procedure; 2) EDIT-INS: Create an incorrect custom block for drawing a polygon because of the wrong usage of ``turn'' blocks. 3) EDIT RUN: Cancel the custom block and run code again without anything drawn. 

We can see that student B runs their program after making one block edit, then they run their program twice after another edit. This is an indicator of debugging behavior with running the program after each single edit. It also suggests that student B does not make progress during the time range when LG1 happens. They move their blocks back-and-forth on stage, which is described as uncertainty or hesitation tinkering behavior by Dong et al. \cite{dong2019defining}, and this is a negative feature of tinkering \cite{perkins1986conditions}. When student B gets stuck, they do not appear to stop and spend time to think over about it or seek help from others. Instead, they act unsystematically, which can make the problem worse \cite{perkins1986conditions}. Beyond student B’s behavior, there are many ways that the pattern LG1 occurs, since it is a general pattern that does not specify block categories. However, it always indicates that a student is running their program frequently within a short period as they enact the pattern. These students may be exhibiting debugging behavior, which has been correlated with lower (B-level) performance \cite{carter2017using}. 


\subsubsection{Case Study 3: Testing Blocks Before Adding}

The LG2 pattern, CHAN RUN EDIT-INS, was detected in assignment A2 as more common among low performers (42\% vs 22\%). The pattern consists of a student changing block categories in Snap, then running some code, and then adding new code. For this pattern, it is important to know that in Snap, students can not only run their whole program (by clicking a ``green flag''), but run individual blocks by clicking on them. This includes blocks in the ``palette'', where students can select blocks in opened categories to be added into their code. Manual inspection of the CHAN RUN pattern revealed that the vast majority of the time, it occurs when students switch to a new category and clicked a block in the palette to run it. In other words, the student was not running \textit{their own} code, but running a block they \textit{could add} to their code. This behavior suggests students are unsure what the block does, and may have been searching for a block with a specific functionality. After running the block, the students would often add it to their code. Interestingly, running these blocks sometimes had no visible effect: for example, a ``repeat'' or ``declare variables'' block has no output when run alone.

As an example, student C engages in the CHAN RUN pattern twice at the start of their session. The student first changes to the \textit{Pen} category, then clicked on the ``pen down'' block in the palette which has no visible effect (i.e. they could not see its output). After 6 seconds, they add it to their code. The student then changes to the \textit{Motion} category and runs a ``move'' block in the palette, which moves the sprite forward. After 3 seconds, they add the ``move'' block to their code as well. While these ``pen down'' and ``move'' blocks are relatively common, it is important to remember that the student has only used these blocks in one prior exercise (A1), so they are still relatively new. This behavior was almost twice as common among low performers on A2, suggesting a hypothesis that testing a block before adding it to their code is an evidence of uncertainty or struggle. In addition to the most common case, described above, LG2 also occurs when students run their custom block by clicking on it in the block palette, rather than by adding it to a script in their own code to run it.

Similar observations have been made in prior work. For example, Zhi et al. \cite{Zhi2019ICER} suggest that Parsons problems -- where students are given all the elements of a correct code solution and must rearrange them -- may be effective in part because students do not waste time identifying the code elements they need to solve a problem. This may be particularly true in block-based programming environments, where students must search for new blocks across a large palette. Our results support this interpretation, and they also suggest that uncertainty about the blocks' functionalities, evidenced by the CHAN RUN pattern, may exacerbate this challenge for novices. Mitrovic et al. \cite{mitrovic2013effect} suggest that programming environments can address this uncertainty with positive feedback, e.g. informing students that they have selected the correct block and made progress.



%\subsection{RQ3}
%From prediction statistics, the CDSM-G performs better on prediction than the CDSM-C among all assignments with higher accuracy and precision across all trials, that means patterns that are more general are more predictive than patterns that are more specific to the programming language context. %Specifically, the average accuracy of CDSM-G is $0.758$ while the average accuracy values of CDSM-C is $0.740$, while the accuracy values ranging in $[0.686, 0.850]$ for CDSM-G and $[0.641, 0.803]$ for CDSM-C. 

% From the case studies, we notice that both general and contextual-specific patterns extracted from our pattern mining can be interpretable, with similar observations made in previous work \cite{wing2006computational, ye1996expert, carter2017using, Zhi2019ICER, mitrovic2013effect}. Besides, context-specific patterns can provide assignment-specific and physical-level insights into students' programs within the block-based programming environment, while general patterns indicate students comprehension on assignments in a more structural and conceptual level.      

==> SIGCSE'21 - Performance Prediction - ArXiv 2/tables/pattern.tex <==


\begin{table*}[t]
\begin{threeparttable}
\caption{Pattern Examples and Corresponding Statistics}
\label{table:pattern}
%\begin{tabular}{lllllll}
\begin{tabular}{p{0.8cm}p{0.8cm}p{9cm}p{1cm}p{1cm}p{0.6cm}p{1.4cm}}
\hline
Index & Ex. & \multicolumn{1}{c}{Patterns}                                                        & PercHigh & PercLow & Diff. & OR \\ \hline
HG1  & A2      & EDIT-INS CHAN EDIT-INS EDIT CHAN EDIT-INS                                           & 52\%     & 31\%    & 21\%  & 2.41       \\
% HC1  & A1      & CHAN-motion EDIT-INS-motion EDIT-motion EDIT-INS-motion EDIT-motion EDIT-INS-motion & 52\%     & 29\%    & 23\%  & 2.65       \\
LG1  & A1      & EDIT-INS EDIT RUN EDIT-INS EDIT RUN                                                 & 37\%     & 60\%    & 23\%  & 0.34       \\ 
LG2 & A2 & CHAN RUN EDIT-INS & 22\% & 42\% & 20\% & 0.39 \\
\hline
\end{tabular}
\begin{tablenotes}
      \small
      \item Ex.: the exercise which the pattern is extracted from; PercHigh/Low: the percentage of high/low-performers who have the pattern; Diff.: difference between PercHigh and PercLow; OR: odds ratio.
    \end{tablenotes}
\end{threeparttable}
\vspace{-0.15 in}
\end{table*}

==> SIGCSE'21 - Performance Prediction - ArXiv 2/tables/predictionResults.tex <==
\begin{table}[t]
\begin{threeparttable}
\small
\caption{Accuracy, Precision, and Recall of the CDSM-based Prediction Models and Baselines}
\label{table:predRes}
%\begin{tabular}{lllllllllllll}
\begin{tabular}{p{0.2cm}p{0.2cm}p{0.2cm}p{0.2cm}p{0.2cm}p{0.2cm}p{0.2cm}p{0.2cm}p{0.2cm}p{0.2cm}p{0.2cm}p{0.2cm}p{0.2cm}}
\hline
                        & \multicolumn{4}{c}{Accuracy}                   & \multicolumn{4}{c}{Precision}                  & \multicolumn{4}{c}{Recall} \\ \hline
\multicolumn{1}{c|}{} & b.1 & b.2 & G    & \multicolumn{1}{c|}{C}    & b.1 & b.2 & G    & \multicolumn{1}{c|}{C}    & b.1  & b.2 & G    & C    \\ %\hline \textit{Ada} \\ \hline
\multicolumn{1}{l|}{M1}   & .509 & .477 & .792 & \multicolumn{1}{l|}{.792} & .509 & .509 & .833 & \multicolumn{1}{l|}{.808} & 1     & .558 & .769 & .808 \\
\multicolumn{1}{l|}{M2}   & .509 & .617 & .773 & \multicolumn{1}{l|}{.753} & .509 & .617 & .759 & \multicolumn{1}{l|}{.741} & 1     & .698 & .830 & .811 \\
\multicolumn{1}{l|}{M3}   & .509 & .677 & .850  & \multicolumn{1}{l|}{.774} & .509 & .684 & .852 & \multicolumn{1}{l|}{.778} & 1     & .722 & .852 & .778 \\
\multicolumn{1}{l|}{M4}   & .509 & .728 & .819 & \multicolumn{1}{l|}{.803} & .509 & .732 & .797 & \multicolumn{1}{l|}{.780} & 1     & .759 & .870 & .852 \\
\multicolumn{1}{l|}{M5}   & .509 & .778 & .803 & \multicolumn{1}{l|}{.784} & .509 & .763 & .770 & \multicolumn{1}{l|}{.746} & 1     & .833 & .870 & .870 \\ \hline

% \textit{Grad} \\ \hline
% \multicolumn{1}{l|}{M1}   & .509                     & .535                     & .755                  & \multicolumn{1}{l|}{.781} & .509                     & .551                     & .750                  & \multicolumn{1}{l|}{.804} & 1                        & .628 & .808                  & .788                  \\
% \multicolumn{1}{l|}{M2}   & .509                     & .594                     & .764                  & \multicolumn{1}{l|}{.745} & .509                     & .596                     & .730                  & \multicolumn{1}{l|}{.755} & 1                        & .721 & .868                  & .755                  \\
% \multicolumn{1}{l|}{M3}   & .509                     & .601                     & .822                  & \multicolumn{1}{l|}{.783} & .509                     & .603                     & .830                  & \multicolumn{1}{l|}{.782} & 1                        & .648 & .815                  & .796                  \\
% \multicolumn{1}{l|}{M4}   & .509                     & .655                     & .809                  & \multicolumn{1}{l|}{.747} & .509                     & .655                     & .783                  & \multicolumn{1}{l|}{.745} & 1                        & .667 & .870                  & .759                  \\
% \multicolumn{1}{l|}{M5}   & .509                     & .620                     & .755                  & \multicolumn{1}{l|}{.791} & .509                     & .349                     & .750                  & \multicolumn{1}{l|}{.767} & 1                        & .500 & .833                  & .852                  \\ \hline

% \textit{RF} \\ \hline
% \multicolumn{1}{l|}{M1}   & .509                     & .390                     & .727                  & \multicolumn{1}{l|}{.727} & .509                     & .415                     & .755                  & \multicolumn{1}{l|}{.736} & 1                        & .423 & .712                  & .750                  \\
% \multicolumn{1}{l|}{M2}   & .509                     & .475                     & .736                  & \multicolumn{1}{l|}{.715} & .509                     & .481                     & .741                  & \multicolumn{1}{l|}{.750} & 1                        & .491 & .755                  & .679                  \\
% \multicolumn{1}{l|}{M3}   & .509                     & .439                     & .784                  & \multicolumn{1}{l|}{.773} & .509                     & .453                     & .804                  & \multicolumn{1}{l|}{.759} & 1                        & .444 & .759                  & .815                  \\
% \multicolumn{1}{l|}{M4}   & .509                     & .614                     & .791                  & \multicolumn{1}{l|}{.765} & .509                     & .627                     & .796                  & \multicolumn{1}{l|}{.738} & 1                        & .593 & .796                  & .833                  \\
% \multicolumn{1}{l|}{M5}   & .509                     & .489                     & .745                  & \multicolumn{1}{l|}{.783} & .509                     & .509                     & .765                  & \multicolumn{1}{l|}{.763} & 1                        & .500 & .722                  & .833                  \\ \hline

% \textit{SVM} \\ \hline
% \multicolumn{1}{l|}{M1}   & .509                     & .498                     & .717                  & \multicolumn{1}{l|}{.715} & .509                     & .519                     & .688                  & \multicolumn{1}{l|}{.722} & 1                        & .519 & .846                  & .750                  \\
% \multicolumn{1}{l|}{M2}   & .509                     & .608                     & .691                  & \multicolumn{1}{l|}{.641} & .509                     & .603                     & .672                  & \multicolumn{1}{l|}{.629} & 1                        & .660 & .774                  & .736                  \\
% \multicolumn{1}{l|}{M3}   & .509                     & .525                     & .755                  & \multicolumn{1}{l|}{.765} & .509                     & .533                     & .712                  & \multicolumn{1}{l|}{.699} & 1                        & .593 & .870                  & .944                  \\
% \multicolumn{1}{l|}{M4}   & .509                     & .538                     & .766                  & \multicolumn{1}{l|}{.737} & .509                     & .537                     & .746                  & \multicolumn{1}{l|}{.717} & 1                        & .667 & .815                  & .796                  \\
% \multicolumn{1}{l|}{M5}   & .509                     & .493                     & .727                  & \multicolumn{1}{l|}{.687} & .509                     & .507                     & .719                  & \multicolumn{1}{l|}{.684} & 1                        & .648 & .759                  & .722                  \\ \hline

% \textit{KNN} \\ \hline
% \multicolumn{1}{l|}{M1}   & .509                     & .479                     & .686                  & \multicolumn{1}{l|}{.707} & .509                     & .491                     & .744                  & \multicolumn{1}{l|}{.717} & 1                        & .519 & .615                  & .731                  \\
% \multicolumn{1}{l|}{M2}   & .509                     & .524                     & .689                  & \multicolumn{1}{l|}{.650} & .509                     & .531                     & .698                  & \multicolumn{1}{l|}{.718} & 1                        & .491 & .698                  & .528                  \\
% \multicolumn{1}{l|}{M3}   & .509                     & .466                     & .728                  & \multicolumn{1}{l|}{.722} & .509                     & .483                     & .821                  & \multicolumn{1}{l|}{.766} & 1                        & .519 & .593                  & .667                  \\
% \multicolumn{1}{l|}{M4}   & .509                     & .578                     & .727                  & \multicolumn{1}{l|}{.699} & .509                     & .571                     & .745                  & \multicolumn{1}{l|}{.677} & 1                        & .667 & .704                  & .778                  \\
% \multicolumn{1}{l|}{M5}   & .509                     & .527                     & .735                  & \multicolumn{1}{l|}{.668} & .509                     & .545                     & .771                  & \multicolumn{1}{l|}{.661} & 1                        & .556 & .685                  & .722                  \\ 
\hline
\end{tabular}
\begin{tablenotes}
      \small
      \item b.1: Majority; b.2: Expert Rule; G: CDSM-G; X: CDSM-C.
    \end{tablenotes}
\label{tab:accuracy}
\end{threeparttable}
\vspace{-0.2in}
\end{table}




==> SIGCSE'21 - Performance Prediction - ArXiv 2/tables/rubric.tex <==
\begin{table*}[t]
\small
\caption{Rubrics of Exercises}
\label{table:rubric}
%\begin{tabular}{|l|l|l|l|l|l|l|}
\begin{tabular}{|p{0.9cm}|p{2.2cm}|p{2.2cm}|p{2.2cm}|p{2.2cm}|p{2.2cm}|p{2.2cm}|}
\hline
Exercise & R1                             & R2                                       & R3                                           & R4                             & R5                                          & R6                                \\ \hline
PM       & code contains 3 block inputs   & set pen thickness                        & repeat \# of required sides                  & move spirit with size length   & turn (\# of sides / 360 degree)             &                                   \\ \hline
SQ       & code contains 1 block input    & set pen down                             & variable initialization                      & repeat rotations for 4 times   & move spirit and turn its direction          & increase counting variable        \\ \hline
GG1      & greet by user's name           & store a random number                    & loop until user guess the correct number     & ask user to guess              & give feedback whether guess is higher/lower & give feedback if guess is correct \\ \hline
GG2      & greet by user's name           & loop until user guess the correct number & give proper feedback to user's guess         & allow user to pick max and min & count number of guesses                     & report number of guesses          \\ \hline
GG3      & allow user to pick max and min & reset list after every game              & loop until spirit guesses the correct number & every new guess is not on list & add guesses to list                         & check whether guess is correct   \\ \hline

\end{tabular}
\end{table*}

==> tables/rubric.tex <==
\begin{table*}[t]
\small
\caption{Rubrics of Exercises}
\label{table:rubric}
%\begin{tabular}{|l|l|l|l|l|l|l|}
\begin{tabular}{|p{0.9cm}|p{2.2cm}|p{2.2cm}|p{2.2cm}|p{2.2cm}|p{2.2cm}|p{2.2cm}|}
\hline
Exercise & R1                             & R2                                       & R3                                           & R4                             & R5                                          & R6                                \\ \hline
PM       & code contains 3 block inputs   & set pen thickness                        & repeat \# of required sides                  & move spirit with size length   & turn (\# of sides / 360 degree)             &                                   \\ \hline
SQ       & code contains 1 block input    & set pen down                             & variable initialization                      & repeat rotations for 4 times   & move spirit and turn its direction          & increase counting variable        \\ \hline
GG1      & greet by user's name           & store a random number                    & loop until user guess the correct number     & ask user to guess              & give feedback whether guess is higher/lower & give feedback if guess is correct \\ \hline
GG2      & greet by user's name           & loop until user guess the correct number & give proper feedback to user's guess         & allow user to pick max and min & count number of guesses                     & report number of guesses          \\ \hline
GG3      & allow user to pick max and min & reset list after every game              & loop until spirit guesses the correct number & every new guess is not on list & add guesses to list                         & check whether guess is correct   \\ \hline

\end{tabular}
\end{table*}
